Data-Driven Operator Theoretic Methods for Phase Space Learning and Analysis

This paper uses data-driven operator theoretic approaches to explore the global phase space of a dynamical system. We defined conditions for discovering new invariant subspaces in the state space of a dynamical system starting from an invariant subspace based on the spectral properties of the Koopman operator. When the system evolution is known locally in several invariant subspaces in the state space of a dynamical system, a phase space stitching result is derived that yields the global Koopman operator. Additionally, in the case of equivariant systems, a phase space stitching result is developed to identify the global Koopman operator using the symmetry properties between the invariant subspaces of the dynamical system and time-series data from any one of the invariant subspaces. Finally, these results are extended to topologically conjugate dynamical systems; in particular, the relation between the Koopman tuple of topologically conjugate systems is established. The proposed results are demonstrated on several second-order nonlinear dynamical systems including a bistable toggle switch. Our method elucidates a strategy for designing discovery experiments: experiment execution can be done in many steps, and models from different invariant subspaces can be combined to approximate the global Koopman operator.

==> Sections/math_prelims.tex <==
\section{Mathematical Preliminaries}
\label{sec:math_prelims}

% \subsection{Notations}
% \begin{tabular}{|c|l|}
% \hline 
% $\pmb\Psi $    & vector valued observable function ($N\times 1$)  \\
% $\phi$ & scalar observable function \\
% $\phi$     & eigenfunction \\
% $\varphi$ & flow operator \\
% $\mathbb{U}$ & infinite dimensional Koopman \\
% ${\cal K}$ & finite dimensional approximation of Koopman \\
% $T$  & discrete-time dynamical system \\
% ${\cal M}$ & State space \\
% $M$ & Invariant subspace \\
% $T_1, T_2$ & Conjugate topological dynamical systems \\
% $h$ & homeomorphism \\
% $\cal B$ & Borel measure \\
% ${\cal G}$ & Functional space (infinite dimensional) \\
% ${\cal G}_{\cal D}$ & Span of $N$ dictionary functions \\
% ${\cal G}^q$ & vector valued dictionary functions ${\cal G} \times \dots \times {\cal G}$ - $q$ times\\
% $\vartheta$ & Koopman modes \\
% $\lambda$ & eigenvalues \\
% $X_p, X_f$ & given datasets \\
% $C^1$ & continuous functions \\
% $x$ & state \\
% $y$ & Equilibrium point \\
% $z$ & Any state \\
% $v$ & number of invariant subspaces \\ 
% $\Phi$ & Null space \\
% \hline 
% \end{tabular}

We recall the necessary concepts that forms a base for the results in this work from \cite{mezic2005spectral,lasota2013chaos,mezic2013analysis,williams2015data,budivsic2012applied}. Consider the following discrete-time nonlinear system
% 
\begin{align}
    x_{t+1} = T(x_t)
    \label{eq:DT_NL_sys}
\end{align}
% 
 where $x \in {\cal M} \subseteq  \mathbb{R}^n$ and $T:{\cal M} \to {\cal M}$. The phase space ${\cal M}$ is assumed to be a compact  manifold with Borel $\sigma$ algebra $\mathcal{B({\cal M})}$, measure $\mu$ \cite{mezic2005spectral,lasota2013chaos} and the nonlinear map $T$ is assumed to be $\mathcal{C}^1$ continuous.  
 
%  

Let $\mathbb{N}$ denote the set of natural numbers. 
% Corresponding to the dynamical system \eqref{eq:DT_NL_sys}, define the flow operator as ${\cal O}: \{\mathbb{N}\cup {0}\} \times {\cal M} \to {\cal M}$ that generates the state trajectory given an initial condition, that is, for any initial condition, $x_0\in {\cal M}$, we obtain $x_t = {\cal O}(t,x_0)$. For brevity, we denote ${\cal O}_t(\cdot) = {\cal O}(t,\cdot)$. 
% 
Recall the definition of invariant set from the classical dynamical systems theory as follows. 
% 
\begin{definition}[Invariant Subspace]
Let $M \subseteq {\cal M}$ be a subspace of the dynamical system, Eq. \eqref{eq:DT_NL_sys}. Then, the subspace $M$ is said to be (positively) invariant if for every $x_0 \in M$, $T^n(x_0) \in M$ for all $n\in\mathbb{N}$.
\end{definition}
% 
Define an observable function on the state space to be a scalar valued function ${\psi}:\mathcal{M} \rightarrow \mathbb{C}$, where $\mathbb{C}$ denotes the set of complex numbers. The scalar valued function ${\psi}$ belongs to the space of functions ${\cal G}$ acting on elements of $\cal M$. Usually for any dynamical system, the output function describes the evolution of the states and this output function can be considered as an observable function. Moreover, any differentiable function of the states can be chosen as an observable function. Normally, square integrable functions defined on ${\cal M}$ forms a good choice of observable functions. Hence, the space of functions, ${\cal G} = L_2({\cal M}, {\cal B}, \mu)$ is infinite dimensional. The Koopman operator can now be defined as follows. 
% 
\begin{definition}[Koopman operator] For a dynamical system $x\mapsto T(x)$ and for ${\psi} \in \mathcal{G}$, the Koopman operator $({\mathbb{U}} : {\cal G} \to {\cal G})$ associated with the dynamical system is defined as
\[ \left[\mathbb{U} {\psi}\right] (x) = \psi(T(x)). \]
\end{definition}
% 

The Koopman operator $\mathbb{U}$ is defined on the space of functions and is a linear operator. The function space ${\cal G}$ is invariant under the action of the Koopman operator. Essentially, instead of studying the time evolution of nonlinear system \eqref{eq:DT_NL_sys} on the state space ${\cal M}$, we study the evolution of \textit{observables} in an infinite dimensional space where the evolution is linear. Apart from being linear, the Koopman operator is also a linear operator: for any $g \geq 0$, $[\mathbb{U} g] (x) \geq 0$.

% also satisfies the following properties:
% \begin{itemize}
% \item Koopman operator is unitary: for any $g \in {\cal G} = L_2({\cal M}, {\cal B}, \mu)$, we obtain, 
% % the Koopman operator $\mathbb{U}: L_2({\cal M}, {\cal B}, \mu) \to L_2({\cal M}, {\cal B}, \mu)$ is unitary, that is, for $g \in {\cal G}$
% % 
% \begin{align*}
%     \parallel \mathbb{U} \; g \parallel^2_\mu= & \int_{\cal M} |g(T(z))|^2d \mu(z) = \int_{\cal M} | g(z)|^2 d\mu(z)=\parallel g\parallel^2_\mu
% \end{align*}
% % 
% and hence all the eigenvalues of $\mathbb{U}$ lie on the unit circle and its eigenfunctions are orthogonal.  
% \item Koopman operator is a positive operator: for any $g \geq 0$, $[\mathbb{U} g] (x) \geq 0$.
% \end{itemize}
% \textcolor{red}{Both the derivations have to be for the vector case. Koopman operator has been defined for a vector of functions, so $\parallel \mathbb{U} g \parallel^2_\mu$ and $g\geq 0$ have to be specified properly. For the first case, I guess we have to use Fubini's theorem because there will be summation to define the norm.}
% 
The infinite dimensional Koopman operator admits discrete and continuous spectrum. In the scope of this work, we are interested in the discrete spectrum of the Koopman operator. The following section describes the popular DMD, EDMD and deepDMD methods to identify a finite dimensional approximate of the Koopman operator from the time-series data. 

% \textcolor{red}{Instead of point spectrum, it is better to use discrete spectrum. I have changes this terminology in the above paragraph.}
